Unveiling the Diversity of Type IIn Supernovae via Systematic Light Curve Modeling

Type IIn supernovae (SNeIIn) are a highly heterogeneous subclass of core-collapse supernovae, spectroscopically characterized by signatures of interaction with a dense circumstellar medium (CSM). Here we systematically model the light curves of 142 archival SNeIIn using MOSFiT (the Modular Open Source Fitter for Transients). We find that the observed and inferred properties of SNIIn are diverse, but there are some trends. The typical SN CSM is dense ($\sim$10$^{-12}$gcm$^{-3}$) with highly diverse CSM geometry, with a median CSM mass of $\sim$1M$_\odot$. The ejecta are typically massive ($\gtrsim10$M$_\odot$), suggesting massive progenitor systems. We find positive correlations between the CSM mass and the rise and fall times of SNeIIn. Furthermore there are positive correlations between the rise time and fall times and the $r$-band luminosity. We estimate the mass-loss rates of our sample (where spectroscopy is available) and find a high median mass-loss rate of $\sim$10$^{-2}$M$_\odot$yr$^{-1}$, with a range between 10$^{-4}$--1M$_\odot$yr$^{-1}$. These mass-loss rates are most similar to the mass loss from great eruptions of luminous blue variables, consistent with the direct progenitor detections in the literature. We also discuss the role that binary interactions may play, concluding that at least some of our SNeIIn may be from massive binary systems. Finally, we estimate a detection rate of 1.6$\times$10$^5$yr$^{-1}$ in the upcoming Legacy Survey of Space and Time at the Vera C. Rubin Observatory.

==> targetlist.tex <==
% \usepackage{tabularx}
% \usepackage{longtable}
% \LTcapwidth=\textwidth
% \usepackage{amsmath}
% \usepackage{pdflscape}

\begin{document}




\begin{landscape}
    \begin{center}
        
    
   % \begin{minipage}{0.99\linewidth}
    
    %\begin{scriptsize}
    \begin{longtable}{lllllll}
    \caption{The full sample of spectroscopically confirmed SNe\,IIn that also have good photometric coverage. This table shows the transient name, the host, discovery date, redshift, J2000 coordinates and the source of the spectrum. The references for each SN is as follows: [1] \citet{2005db},[2] \citet{2006gy}, [3] \citet{Ransome_2021}, [4] \citet{1998s}, [5] \citet{1994y} [6] \citet{1995n} [7] \citet{2008b} [8] \citet{2018fdt_disc} [9] \citet{2018fdt_spec}, [10] \citet{2018khn_disc}, [11] \citet{2018khn_spec}, [12] \citet{2018kyv_disc}, [13] \citet{2018kyv_spec}, [14] \citet{2018leh_disc}, [15] \citet{2018leh_spec}, [16] \citet{2019bxq_disc}, [17] \citet{2019bxq_spec}, [18] \citet{2019dvv_disc}, [19] \citet{2019dvv_spec}. [20] \citet{2019gjs_disc}, [21] \citet{2019gjs_spec}, [22] \citet{2019hgy_disc}, [23] \citet{2019hgy_spec}, [24] \citet{2019krt_disc}, [25] \citet{2019krt_spec}, [26] \citet{2019lkr_disc}, [27] \citet{2019lkr_spec}, [28] \citet{2019pgu_disc}, [29] \citet{2019pgu_spec}, [30] \citet{2019qny_disc}, [31] \citet{2019qny_spec}, [32] \citet{2019qt_disc}, [33] \citet{2019qt_spec}, [34] \citet{2019qvr_disc}, [35] \citet{2019qvr_spec}, [36] \citet{2019rz_disc}, [37] \citet{2019rz_spec}, [38] \citet{2019sxv_disc}, [39] \citet{2019sxv_spec}, [40] \citet{2019vkl_disc}, [41] \citet{2019vkl_spec}, [42] \citet{2019wmf_disc}, [43] \citet{2019wmf_spec}, [44] \citet{2019wnc_disc}, [45] \citet{2019wnc_spec}, [46] \citet{2020aafb_disc}, [47] \citet{2020aafb_spec}, [48] \citet{2020aaut_disc}. [49] \citet{2020aaut_spec}, [50] \citet{2020cn_disc}, [51] \citet{2020cn_spec}, [52] \citet{2020fhw_disc}, [53] \citet{2020fhw_spec}. [54] \citet{2020hem_disc}, [55] \citet{2020hem_spec}, [56] \citet{2020rc_disc}, [57] \citet{2020rc_spec}, [58] \citet{2020rno_disc}, [59] \citet{2020rno_spec}, [60] \citet{2020sj_disc}, [61] \citet{2020sj_spec}, [62] \citet{2020tis_disc}, [63] \citet{2020tis_spec}, [64] \citet{2020tyk_disc}, [65] \citet{2020tyk_spec}, [66] \citet{2020vci_disc}, [67] \citet{2020vci_spec}, [68] \citet{2020vou_disc}, [69] \citet{2020vou_spec}, [70] \citet{2020xpo_disc}, [71] \citet{2020xpo_spec}, [72] \citet{2020yy_disc}, [73] \citet{2020yy_spec}, [74] \citet{2020zos_disc}, [75] \citet{2020zos_spec}, [76] \citet{2021bwf_disc}, [77] \citet{2021bwf_spec}, [78] \citet{2021bxo_disc}, [79] \citet{2021bxo_spec}, [80] \citet{2021ezt_disc}, [81] \citet{2021ezt_spec}, [82] \citet{2021fel_disc}, [83] \citet{2021fel_spec}, [84] \citet{2021fpn_disc}, [85] \citet{2021fpn_spec}, [86] \citet{2021gpw_disc}, [87] \citet{2021gpw_spec}, [88] \citet{2021hur_disc}, [89] \citet{2021hur_spec}, [90] \citet{2021hsn_disc}, [91] \citet{2021hsn_spec}, [92] \citet{2021iui_disc}, [93] \citet{2021iui_spec}, [94] \citet{2021kat_disc}, [95] \citet{2021kat_spec}, [96] \citet{2021kqv_disc}, [97] \citet{2021kqv_spec}, [98] \citet{2021kwc_disc}, [99] \citet{2021kwc_spec}, [100] \citet{2021kwj_disc}, [101] \citet{2021kwj_spec}, [102] \citet{2021lhy_disc}, [103] \citet{2021lhy_spec}, [104] \citet{2021osr_disc}, [105] \citet{2021osr_spec}, [106] \citet{2021qeq_disc}, [107] \citet{2021qeq_spec}, [108] \citet{2021qug_disc}, [109] \citet{2021qug_spec}, [110] \citet{2021srg_disc}, [111] \citet{2021srg_spec}, [112] \citet{2021ukt_disc}, [113] \citet{2021ukt_spec}, [114] \citet{2021uru_disc}, [115] \citet{2021uru_spec}, [116] \citet{2021vzp_disc}, [117] \citet{2021vzp_spec}, [118] \citet{2021wrr_disc}, [119] \citet{2021wrr_spec}, [120] \citet{2021yaz_disc}, [121] \citet{2021yaz_spec} [122] \citet{2021ydc_disc}, [123] \citet{2021ydc_spec}, [124] \citet{2021yys_disc}, [125] \citet{2021yys_spec}, [126] \citet{2021yyy_disc}, [127] \citet{2021yyy_spec}, [128] \citet{2021ras_disc}, [129] \citet{2021ras_spec}, [130] \citet{2022fnl_disc}, [131] \citet{2022fnl_spec}, [132] \citet{2022jie_disc}, [133] \citet{2022jie_spec}, [134] \citet{2022mds_disc}, [135] \citet{2022mds_spec}, [136] \citet{2022mma_disc}, [137] \citet{2022mma_spec}, [138] \citet{2022mma_disc}, [139] \citet{2022mma_spec}, [140] \citet{2022myl_disc}, [141] \citet{2022myl_spec}, [142] \citet{2022oeh_disc}, [143] \citet{2022oeh_spec}, [144] \citet{2022paz_disc}, [145] \citet{2022paz_spec}, [146] \citet{2022prr_disc}, [147] \citet{2022prr_spec}, [148] \citet{2022pss_disc}, [149] \citet{2022pss_spec}, [150] \citet{2022rhl_dsic}, [151] \citet{2022rhl_spec}, [152] \citet{2022tbh_disc}, [153] \citet{2022tbh_spec}, [154] \citet{2022ymc_disc}, [155] \citet{2022ymc_spec}, [156] \citet{2022zyd_disc}, [157] \citet{2022zyd_spec}, [158] \citet{2023adz_disc}, [159] \citet{2023adz_spec}, [160] \citet{2023awp_disc}, [161] \citet{2023awp_spec}, [162] \citet{2023erg_disc}, \citet{2023erg_spec}, [164] \citet [34] \citet{Nyholm_2020} and [35] \citet{Villar_2020}. 
    \textit{* as presented in \citet{Ransome_2021}.} 
    \label{tab:sample}} 
    
    \hline
    %Name & Disc. Date & Host Name & R.A. & Dec. & $z$ &OSC &TNS& SNID &Class&Source\\
    SN Name & Host & Host type & $z$ & R.A (J2000) & Dec (J2000)  & Ref. \\
    \hline
    \endfirsthead
    \multicolumn{7}{l}{\tablename\ \thetable\ --- Continued from previous page\ldots}\\
    \hline
    %Name & Disc. Date & Host Name & R.A. & Dec. & $z$ &OSC &TNS& SNID &Class&Source\\
    SN Name & Host & Host type & $z$ & R.A (J2000) & Dec (J2000) & Ref. \\
    \hline
    \endhead
    \hline
    \endlastfoot
    \hline
    \multicolumn{7}{r}{Continued on next page\ldots}\\
    \endfoot
    
            SN\,2005db & NGC\,214& Sbc & 0.0151 & 00:41:26.79 & 25:29:51.60  & \citet{2005db} \\
            SN\,2006gy & NGC\,1260& SB0a & 0.0192 & 03:17:27.06 & 41:24:19.51  & \citet{2006gy}  \\
            SN\,1989C & MCG+01-25-25& SB & 0.0063 & 09:47:45.49 & 02:37:36.10  & P.~Challis*\\
            SN\,1998S &  NGC\,3877& SA & 0.0030 & 11:46:06.13 & 47:28:55.40  & \citet{1998s} \\
            SN\,1994W & NGC\,4041& SAB &  0.00403 & 12:02:10.92 & 62:08:32.70  & \citet{Ransome_2021}  \\
            SN\,1994Y & NGC\,5371& SABbc & 0.0085  & 13:55:36.90 & 40:27:53.40  &\citet{1994y} \\
            SN\,1995N & MCG-02-38-17& IB & 0.0062  & 14:49:28.29 & -10:10:14.40  & \citet{1995n} \\
            SN\,2008B & NGC\,5829& - & 0.0188 & 15:02:43.65 & 23:20:07.80  & \citet{2008b} \\
            \hline
            SN\,2018fdt &Z\,197-30& SBc & 0.0550 & 17:04:44.33 & +38:14:08.0 &  \citet{2018fdt_disc}, \citet{2018fdt_spec} \\
            SN\,2018khn & WISEA\,J085619.17+523252.7& -& 0.0910 & 08:56:18.01 & +52:32:58.00   & \citet{2018khn_disc}, \citet{2018khn_spec} \\
            SN\,2018kyv & WISEA\,J130104.80+262103.2& - &  0.0940 & 13:01:04.95& +26:21:03.8 & \citet{2018kyv_disc}, \citet{2018kyv_disc} \\
            SN\,2018leh & UGC\,2949& SB:ab & 0.02396 &04:05:03.30 & +25:15:42.90   & \citet{2018leh_disc}, \citet{2018leh_spec}\\
            SN\,2019bxq & 2MASX\,J16575851+7836144& E & 0.0140 &16:57:58.51 & +78:36:13.6 &  \citet{2019bxq_disc}, \citet{2019bxq_spec}\\
            SN\,2019dvv & LEDA\,89698& S & 0.0305 & 12:23:17.77 & +19:43:23.3	 & \citet{2019dvv_disc}, \citet{2019dvv_spec}\\
            SN\,2019gjs & UGC\,9634& Sb & 0.0430 &  14:58:57.16& +20:03:10.50  &\citet{2019gjs_disc}, \citet{2019gjs_spec}\\
            SN\,2019hgy & WISEA\,J174820.57+481206.9& -  & 0.0360 &17:48:20.50  & +48:12:07.0 &\citet{2019hgy_disc}, \citet{2019hgy_spec}\\
            SN\,2019krt & SDSS\,J165256.08+204305.6& -& 0.0300 &16:52:54.76 &+20:43:03.5&\citet{2019krt_disc}, \citet{2019krt_spec} \\
            SN\,2019lkr & LEDA\,2756618&-& 0.0300 & 16:05:07.98& +73:35:04.0 & \citet{2019lkr_disc}, \citet{2019lkr_spec} \\
            SN\,2019pgu & -  &- & 0.1055 &	16:18:42.83 & +67:54:00.30 &\citet{2019pgu_disc}, \citet{2019pgu_spec} \\
            SN\,2019qny & LEDA\,1083065& - & 0.0480 & 03:32:59.94 & -02:46:41.50 & \citet{2019qny_disc}, \citet{2019bxq_spec} [31] \\
            SN\,2019qt & - &- & 0.0350 & 	14:59:10.65 & +43:49:11.60 & \citet{2019qt_disc}, \citet{2019qt_spec} \\
            SN\,2019qvr & - & - & 0.0750 & 	03:41:21.69 & +22:49:20.80 & \citet{2019qvr_disc}, \citet{2019qvr_spec} \\
            SN\,2019rz & UGC\,3445& SB:b & 0.01885 & 06:50:25.81 & +43:03:11.60 & \citet{2019rz_disc}, \citet{2019rz_spec} \\
            SN\,2019sxv & 2MASX\,J22195786+2537447& - & 0.0400 & 22:19:58.25 & +25:37:46.7  &\citet{2019sxv_disc}, \citet{2019sxv_spec} \\
            SN\,2019vkl & WISEA\,J015630.94+182623.5& - & 0.0640 &01:56:30.79  & +18:26:23.8 &\citet{2019vkl_disc}, \citet{20219vkl_spec} \\
            SN\,2019wmf & WISEA\,J102954.55+704710.0& - & 0.0600 & 10:29:53.88& +70:47:09.60 &\citet{2019wmf_disc}, \citet{2019wmf_spec} \\
            SN\,2019wnc & LEDA\,1183665& - & 0.0216 & 10:10:56.36 & +01:04:17.10 &\citet{2019wnc_disc}, \citet{2019wnc_spec} \\
            SN\,2020aafb & WISEA\,J015128.98+224947.2& - & 0.0780 & 01:51:28.95 & +22:49:44.10 &\citet{2020aafb_disc}, \citet{2020aafb_spec}\\
            SN\,2020aaut & LEDA\,1221074& - & 0.0757 & 12:09:12.54 & +02:15:24.3 & \citet{2020aaut_disc}, \citet{2020aaut_spec}\\
            SN\,2020cn & - & - & 0.0770 & 21:28:10.73 & +79:06:36.30 & \citet{2020cn_disc}, \citet{2020cn_spec} \\
            SN\,2020fhw & WISEA\,J150029.88+171410.8& - & 0.1116 & 15:00:29.89 & +17:14:10.50 & \citet{2020fhw_disc}, \citet{2020fhw_spec} \\
            SN\,2020hem & 2MASX\,J15024011+0918137& - & 0.0935 & 15:02:40.15 & +09:18:13.8 & \citet{2020hem_disc}, \citet{2020hem_spec} \\
            SN\,2020rc & - & - & 0.0810 & 11:50:34.07 & -04:20:22.7 & \citet{2020rc_disc}, \citet{2020rc_spec} \\
            SN\,2020rno & - & - & 0.0640 & 01:18:51.79 & +18:40:09.50 &\citet{2020rno_disc}, \citet{2020rno_spec} \\
            SN\,2020sj & - & - & 0.0770 & 09:26:19.87 & -07:28:30.00 &\citet{2020sj_disc}, \citet{2020sj_spec} \\
            SN\,2020tis & WISEA\,J235725.57+250330.7& - & 0.0577 & 23:57:24.78 & +25:03:48.6 &\citet{2020tis_disc}, \citet{2020tis_spec} \\
            SN\,2020tyk & - & - & 0.0870 & 01:37:58.38 & +20:00:03.00 &\citet{2020tyk_disc}, \citet{2020tyk_spec} \\
            SN\,2020vci & - & -  & 0.1930 & 15:04:22.63& +51:04:56.80 &\citet{2020vci_disc}, \citet{2020vci_spec} \\
            SN\,2020vou & WISEA\,J233743.84+215110.8& - & 0.1190 & 23:37:43.80 & +21:51:14.60 &\citet{2020vou_disc}, \citet{2020vou_spec} \\
            SN\,2020xpo & GALEXASC\,J023225.46-125741.7& - & 0.0750 & 02:32:25.65 & -12:57:41.00&\citet{2020xpo_disc}, \citet{2020xpo_spec} \\
            SN\,2020yy & SDSS\,J141853.90+630945.& - & 0.0675 & 14:18:53.91 & +63:09:45.00 &\citet{2020yy_disc}, \citet{2020yy_spec}\\
            SN\,2020zos & WISEA\,J050632.07+074535.3& - & 0.1400 & 05:06:32.08 & +07:45:36.40 &\citet{2020zos_disc}, \citet{2020zos_spec} \\
            SN\,2021bwf & SDSS\,J163457.25+562855.8& - & 0.1940 & 16:35:02.9 & +56:28:38.40 &\citet{2021bwf_disc}, \citet{2021bwf_spec}\\
            SN\,2021bxo & Mrk\,1209Ê& Sp & 0.0339 & 08:04:00.58 & +10:00:33.5 &\citet{2021bxo}, \citet{2021bxo_spec} \\
            SN\,2021ezt & 2MASX\,J16583923+2629311& - & 0.05016 & 16:58:38.98 & +26:29:32.4  & \citet{2021ezt_disc}, \citet{2021ezt_spec}\\
            SN\,2021fel & WISEA\,J165158.55+623404.8& - & 0.0680 & 16:51:58.52 & +62:34:04.30  &\citet{2021fel_disc}, \citet{2021fel_spec}\\
            SN\,2021fpn & ZwCl\,1012-0047&- & 0.0424 & 10:13:47.65&	-00:54:55.00  &\citet{2021fpn_disc}, \citet{2021fpn_spec} \\
            SN\,2021gpw & WISEA\,J132154.84+164439.7&- & 0.0750 & 13:21:54.85&	+16:44:39.70  &\citet{2021gpw_disc}, \citet{2021gpw_spec}\\
            SN\,2021hur & LEDA 2773190& - & 0.0300 & 13:30:59.36 &	+77:12:52.60  &\citet{2021hur_disc}, \citet{2021hur_spec}\\
            SN\,2021hsn & - &- & 0.0540 & 19:22:16.83&	+56:21:00.20 & \citet{2021hsn_disc}, \citet{2021hsn_spec}\\
            SN\,2021iui & SDSS\,J141659.24+321406.7& - & 0.1060 & 14:16:59.19 & +32:14:06.5 &\citet{2021iui_disc}, \citet{2021iui_spec} \\
            SN\,2021kat & - & - & 0.1013 & 19:50:31.65 & +57:59:28.00 &\citet{2021kat_disc}, \citet{2021kat_spec} \\
            SN\,2021kqv & UGC\,10132& SB:b & 0.0510 & 15:56:52.03 & +78:27:48.9 &\citet{2021kqv_disc}, \citet{2021kqv_spec} \\
            SN\,2021kwc & NGC\,5231& SA & 0.02175 &13:35:47.91 & +02:59:59.30 &\citet{2021kwc_disc}, \citet{2021kwc_spec}\\
            SN\,2021kwj & WISEA\,J181949.35+561011.3& - & 0.0250 &18:19:49.50 & +56:10:01.20 &\citet{2021kwj_disc}, \citet{2021kwj_spec} \\
            SN\,2021lhy & WiggleZ\,R22J213215370-00310110&- & 0.1420 & 21:32:14.94	&-00:30:05.10  &\citet{2021lhy_disc}, \citet{2021lhy_spec} \\
            SN\,2021osr & 2MASX\,J21345199-0726529& -& 0.08545 & 21:34:51.91&	-07:26:54.5  & \citet{2021osr_disc}, \citet{2021osr_spec}\\
            SN\,2021qeq & - &- & 0.0550 &  16:54:26.77&	+53:43:26.3 &\citet{2021qeq_disc}, \citet{2021qeq_spec}\\
            SN\,2021qug & J220232.70-164537.8&- & 0.0570 & 22:02:32.45	&-16:45:36.4  &\citet{2021qug_disc}, \citet{2021qug_spec}\\
            SN\,2021ras & 2MASX\,J17385176+2622447&- & 0.0290 & 17:38:51.92& 	+26:22:44.20  &\citet{2021ras_disc}, \citet{2021ras_disc} \\
            SN\,2021srg & WISEA\,J231817.23+145004.& -& 0.0690 &23:18:17.26	&+14:50:04.80  &\citet{2021srg_disc}, \citet{2021srg_spec}\\
            SN\,2021ukt & UGC\,505& S & 0.01288 & 00:49:24.86&	-01:45:58.70  & \citet{2021ukt_disc}, \citet{2021ukt_spec}\\
            SN\,2021uru & LEDA\,864812& - & 0.0540 &02:52:22.67&	-18:41:47.50  &\citet{2021uru_disc}, \citet{2021uru_spec}\\
            SN\,2021vzp & 2MASX\,J03473546+0252586& - & 0.0310 &03:47:35.55&	+02:52:58.40 &\citet{2021vzp_disc}, \citet{2021vzp_spec}\\
            SN\,2021wrr & WISEA\,J171107.70+722919.8& - & 0.0480 & 17:11:07.79	&+72:29:19.80 &\citet{2021wrr_disc}, \citet{2021wrr_spec} \\
            SN\,2021yaz & - & -& 0.0390 &02:30:37.00 &+25:26:07.50  & \citet{2021yaz_disc}, \citet{2021yaz_spec} \\
            SN\,2021ydc & WISEA\,J012517.64+222324.8&- &0.0550&01:25:17.62 &	+22:23:25.30 &\citet{2021ydc_disc}, \citet{2021ydc_spec}\\
            SN\,2021yys & 2MASX\,J07254250+4449209&- & 0.04329 & 07:25:42.21 & +44:49:25.10 &\citet{2021yys_disc}, \citet{2021yys_spec} \\
            SN\,2021yyy & WISEA\,J224007.46-050012.4&- &0.0930 &22:40:07.55	&-05:00:12.50   &\citet{2021yyy_class}, \citet{2021yyy_spec} \\
            SN\,2022fnl & WISEA\,J153342.47+434445.5&- & 0.1035 & 15:33:42.47&	+43:44:45.40  &\citet{2022fnl_disc}, \citet{2022fnl_spec} \\
            SN\,2022jie & LEDA\,2669503& - & 0.0748 & 12:42:48.12	&+64:34:29.60  & \citet{2022jie_disc}, \citet{2022jie_spec} \\
            SN\,2022mds & WISEA\,J173233.61+431623.3& -& 0.0745 &17:32:33.90&	+43:16:27.10  &\citet{2022mds_disc}, \citet{2022mds_spec} \\
            SN\,2022mma & Z\,104-58& Sc & 0.0380 & 14:39:01.49	&+15:59:11.70 & \citet{2022mma_disc}, \citet{2022mma_spec}\\
            SN\,2022myl & Z\,169-7& - & 0.0371 & 16:51:02.37 &	+30:39:52.30 & \citet{2022myl_disc}, \citet{2022myl_spec} \\
            SN\,2022oeh & LEDA\,2273049&- & 0.0300 & 19:16:50.01&	+45:57:18.60 & \citet{2022oeh_disc}, \citet{2022oeh_spec}\\
            SN\,2022paz & - & -& 0.0660 &18:05:09.01&	+32:09:00.90  &\citet{2022paz_disc}, \citet{2022paz_spec}\\
            SN\,2022prr & NGC\,6745& -& 0.0152& 19:01:41.90& +40:45:03.70  & \citet{2022prr_disc}, \citet{2022prr_spec}\\
            SN\,2022pss & - & -& 0.0600 & 01:28:19.22	&+20:23:45.30  & \citet{2022pss_disc}, \citet{2022pss_spec} \\
            SN\,2022rhl & - &- & 0.1180 & 19:20:44.21 & +46:52:54.70 & \citet{2022rhl_dsic}, \citet{2022rhl_spec} \\
            SN\,2022tbh & LEDA 2706824 & - & 0.0520 & 17:25:09.72 & +67:49:45.77 & \citet{2022tbh_disc}, \citet{2022tbh_spec} \\
            SN\,2022ymc & - &- & 0.0280 & 03:13:40.62 & -01:16:32.21 & \citet{2022ymc_disc}, \citet{2022ymc_spec} \\
            SN\,2022zyd & - &- & 0.0630& 02:08:33.20 & +52:49:36.37 & \citet{2022zyd_disc}, \citet{2022zyd_spec} \\
            SN\,2023adz & - &- & 0.0500 & 11:32:37.72 & +68:23:48.74 & \citet{2023adz_disc}, \citet{2023adz_spec} \\
            SN\,2023awp & NGC\,5936 &Sc & 0.0136 & 15:30:01.54  & +12:59:15.56 & \citet{2023awp_disc}, \citet{2023awp_spec} \\
            SN\,2023erg & - &- & 0.0670 & 15:30:05.64 & +35:40:19.92 & \citet{2023erg_disc}, \citet{2023erg_spec} \\
            SN\,2023iex & 2MASX\,J21395531+2439332 &- & 0.0290 & 21:39:56.07  &  +24:39:34.67 & \citet{2023iex_disc}, \citet{2023iex_spec} \\
            SN\,2023kqw & SDSS\,J143643.35+120523.8 &- & 0.0547 & 14:36:43.33 &  +12:05:24.26 & \citet{2023kqw_disc}, \citet{2023kqw_spec} \\
            SN\,2023meo & SDSS\,J143643.35+120523.8 &- & 0.054 & 21:40:59.12 & +24:00:26.28 & \citet{2023meo_disc}, \citet{2023meo_spec} \\
            SN\,2023nof & 2dFGRS\,TGS855Z331 &- & 0.0692 & 22:39:44.18 &  -15:50:04.38 & \citet{2023nof_disc}, \citet{2023nof_spec} \\
            SN\,2023pfj & - &- & 0.1110 & 02:17:12.15 & +01:35:56.35 & \citet{2023pfj_disc}, \citet{2023pfj_spec} \\
            SN\,2023usc & - &- & 0.0600 & 05:21:31.65  &  +00:28:20.72 & \citet{2023usc_disc}, \citet{2023usc_spec} \\
            \hline
            SN\,2019uit & NGP9\,F378-0626697&- & 0.0710 & 12:50:16.09& +21:20:15.40 & \citet{2019uit_disc}, \citet{2019uit_spec} \\
            SN\,2020jhs & - & -& 0.0650 & 09:28:14.09& +25:40:13.30 & \citet{2020jhs_disc},\citet{2020jhs_spec} \\
            SN\,2020qmj & LEDA\,1280605&- & 0.0220 & 00:44:06.006 &+05:15:35.93  & \citet{2020qmj_disc}, \citet{2020qmj_spec} \\
            SN\,2020tan & SDSS\,J010944.57+002024.3& -& 0.0790 &01:09:44.599& +00:20:24.93 & \citet{2020tan_disc}, \citet{2020tan_spec} \\
            SN\,2020uaq & SDSS\,J153452.65+105839.1& -& 0.1150 & 15:34:49.030& +10:58:37.34 & \citet{2020uaq_disc}, \citet{2020uaq_spec}\\
            SN\,2020utm & LEDA\,1078124&	- & 0.0440 & 03:15:27.45 &-03:00:38.19 &\citet{2020utm_disc}, \citet{2020utm_spec}\\
            SN\,2020ybn & - & -& 0.0960 & 06:11:02.260& -22:17:50.28  &\citet{2020ybn_disc}, \citet{2020ybn_spec} \\
            SN\,2021aapa & MCG-02-11-023  & - & 0.0320 & 22:04:24.170 &-19:32:28.63 & \citet{2021aapa_disc}, \citet{2021aapa_spec}\\
            \hline
            iPTF\,13agz & SDSS\,J143432.09+250941.5& - &0.05715 &14 34 32.12 &+25 09 43.60 & [34]\\
            iPTF\,13asr & - & -& 0.15427 &12:47:28.61&	+27:04:03.60 &  [34]\\
            iPTF\,13cuf & - &- & 0.21994 &02:04:52.97&	+14:37:59.7  &  [34]\\
            iPTF\,14bpa & - &- & 0.12197 & 15:26:59.96&	+24:41:17.5&   [34]\\
            iPTF\,15aym & MCG+09-22-059& -&0.03344 &13 26 26.67&	+55 23 43.40  & [34]\\
            iPTF\,15bky & NGC\,5837& E &0.02877 &15 04 40.80	&+12 37 43.40 & [34]\\
            iPTF\,15blp & - & -& 0.19486 &16 27 15.21&	+41 08 58.10  & [34] \\
            iPTF\,15eqr & WISEA\,J040115.10+331700.1& -& 0.04671&04 01 15.67&	+33 16 58.30 & [34]\\
            iPTF\,16fb & WISEA\,J102209.12+152822.4& -& 0.08112&10 22 09.25	&+15 28 19.2  & [34]\\
            PTF\,10abui & - & -& 0.05162&06 12 18.46	&-22 46 15.6 & [34]\\
            PTF\,10acsq & SDSS\,J080133.14+464553.0& - &0.17303 & 08 01 33.17	&+46 45 52.5 & [34] \\
            PTF\,10cwl & - & -& 0.08489& 12 36 22.06&	+07 47 38.0 &[34] \\
            PTF\,10cwx & 2dFGRS\,TGN321Z210 &- &0.07312 &12 33 16.53&	-00 03 10.6 & [34] \\
            PTF\,10ewc & - & -& 0.05424 &14 01 59.08&	+33 50 11.6  &[34] \\
            PTF\,10fjh & UGC\,10547 & SAb & 0.03209 &16 46 55.36	&+34 09 34.70 & [34] \\
            PTF\,10flx & WISEA\,J164658.92+642650.0&- & 0.06744 &16 46 58.28&	+64 26 48.50 & [34] \\
            PTF\,10gvd & - & -& 0.06928 &16 53 02.12&	+67 00 08.9  &[34]\\
            PTF\,10gvf & SDSS\,J111344.87+533749.6&- & 0.08092 &11 13 45.24&	+53 37 44.90& [34] \\
            PTF\,10oug & - & -& 0.15007 &17 20 44.79&	+29 04 25.6 &[34] \\
            PTF\,10qwu & - &- & 0.22585 &16 51 10.36&	+28 18 06.2 & [34]\\
            PTF\,10tel & A\,J172130+4807& -& 0.03487 & 17 21 30.68	&+48 07 47.40& [34]\\
            PTF\,10tyd & LEDA\,1818789&	- & 0.06325 &17 09 19.41	&+27 49 08.6 & [34] \\
            PTF\,10weh & - & -& 0.13788 & 17 26 50.46	&+58 51 07.4 & [34]\\
            PTF\,11fzz & - & -& 0.08132 &11 10 46.68&	+54 06 18.80 & [34]\\
            PTF\,11oxu & WISEA\,J033834.32+223242.7& - & 0.08780 &03:38:34.38&	+22:32:59.4 &[34]\\
            \hline
            PSc\,130812 & - &- &0.0141 &12:22:32.93    &	+47:19:48.36& [35] \\
            PSc\,130942 & - &- &0.0087&16:01:26.26     &	+55:14:25.80 & [35] \\
            PSc\,150582  & - & -& 0.0099&10:47:16.30    &	+59:01:26.04 & [35] \\
            PSc\,300140  & - &- &0.0406& 23:30:48.91    &	-01:12:26.64 & [35] \\
            PSc\,350633 & - & -&0.0059 & 10:45:19.15    &	+59:04:54.84  & [35] \\
            PSc\,430005 & - & -& 0.0564&22:17:39.86    	&+00:37:35.40  & [35] \\
            PSc\,450025 & - & -&0.0237&02:23:33.53    	&-05:32:01.68  & [35] \\
            PSc\,450266  & - & -& 0.0259& 08:40:55.46      &	+44:56:41.64   & [35] \\
            PSc\,460001  & - & -& 0.0077& 03:33:04.15    &-28:12:49.32  & [35] \\
            PSc\,480845 & - & - &0.0135 &12:29:08.59       &	+46:52:47.28   & [35] \\
            PSc\,500063 & - & - & 0.0118&12:25:06.67  &	+47:55:33.96  & [35] \\
            PSc\,530085 & - & - &0.0661 & 22:12:43.46  &-00:05:07.44 & [35] \\
            PSc\,550221  & - & - &0.0243 & 02:21:52.39    &	-03:26:00.60  & [35] \\
            PSc\,580280 & - & - &0.0074 &03:32:54.12& -28:14:24.00 & [35] \\
            PSc\,580280 & - & - &0.0373 &02:28:34.32    	&-04:54:46.08   & [35] \\  
    
    
    \end{longtable}
%    \end{scriptsize}
%    \end{minipage}
    \end{center}
\end{landscape}

\end{document}
